The Bias-Expressivity Trade-off

Learning algorithms need bias to generalize and perform better than random guessing. We examine the flexibility (expressivity) of biased algorithms. An expressive algorithm can adapt to changing training data, altering its outcome based on changes in its input. We measure expressivity by using an information-theoretic notion of entropy on algorithm outcome distributions, demonstrating a trade-off between bias and expressivity. To the degree an algorithm is biased is the degree to which it can outperform uniform random sampling, but is also the degree to which is becomes inflexible. We derive bounds relating bias to expressivity, proving the necessary trade-offs inherent in trying to create strongly performing yet flexible algorithms.

==> futility-results.tex <==
    \begin{restatable}[Improbability of Favorable Information Resources]{theorem}{iofir}
        Let $\mathcal{D}$ be a distribution over a set of information resources $\mathcal{F}$, let $F$ be a random variable such that $F \sim \mathcal{D}$, let $t \subseteq \Omega$ be an arbitrary fixed $k$-sized target set with corresponding target function $\bm{t}$, and let $q(t,F)$ be the expected per-query probability of success for algorithm $\mathcal{A}$ on search problem $(\Omega,t,F)$. Then, for any $q_{\mathrm{min}} \in [0,1]$,
        \begin{align*}
            \Pr(q(t, F) \geq q_\mathrm{min})  &\leq \frac{p + \bias(\mathcal{D}, \bm{t})}{q_{\mathrm{min}}}
        \end{align*}
        where $p = \frac{k}{|\Omega|}$.
        \label{thm:iofir}
    \end{restatable}
    \noindent
    Since the size of the target set $t$ is usually small relative to the size of the search space $\mathrm{\Omega}$, $p$ is also usually small. Following the above results, we see that the probability that a search problem with an information resource drawn from $\mathcal{D}$ is favorable is bounded by a low value. This bound tightens as we increase our minimum threshold of success, $q_\mathrm{min}$. Notably, our bound relaxes with the introduction of bias. 
    
    \begin{restatable}[Probability of Success Under Bias-Free Search]{corollary}{reducedprob}
    When \(\bias(\mathcal{D}, \bm{t}) = 0\),
    \begin{align*}
        \Pr(q(t, F) \geq q_\mathrm{min}) &\leq \frac{p}{q_{\mathrm{min}}}
    \end{align*}
    \end{restatable}
    \noindent Directly following Theorem~\ref{thm:iofir}, if the algorithm does not induce bias on $\bm{t}$ given a distribution over a set of information resources, the probability of successful search by a favorable information resource cannot be any higher than that of uniform random sampling divided by the minimum performance that we specify. 
    
    \begin{restatable}[Geometric Divergence]{corollary}{geometricdivergence}
    \begin{align*}
              \Pr(q(t, F) \geq q_\mathrm{min}) &\leq \frac{\sqrt{k} \cos (\theta)}{q_{\mathrm{min}}} 
              = \frac{\| \bm{t} \| \cos (\theta)}{q_{\mathrm{min}}}
         \end{align*}
    \end{restatable}
    \noindent
     This result shows that greater geometric alignment between the target vector and expected distribution over the search space loosens the upper bound on the probability of successful search. Connecting this to our other results, the geometric alignment can be viewed as another interpretation of the bias the algorithm places on the target set.
    
    \begin{restatable}[Conservation of Bias]{theorem}{conservation}
    Let $\mathcal{D}$ be a distribution over a set of information resources and let $\tau_{k} = \{ \bm{t} | \bm{t} \in \{ 0, 1 \}^{ |\Omega| }, ||\bm{t}|| = \sqrt{k} \}$ be the set of all $|\Omega|$-length $k$-hot vectors. Then for any fixed algorithm $\mathcal{A}$, 
    \begin{align*}
        \sum_{\bm{t} \in \tau_{k}} \bias(\mathcal{D},\bm{t}) = 0
    \end{align*}
    \label{thm:consbias}
    \end{restatable}
    \noindent
    Since bias is a conserved quantity, an algorithm that is biased towards any particular target is equally biased against other targets, as is the case in Schaffer's conservation law for generalization performance~\cite{schaffer1994conservation}. This conservation property holds regardless of the algorithm or the distribution over information resources. Positive dependence between targets and information resources is the grounds for all successful machine learning~\cite{montanez2017dissertation}, and this conservation result is another manifestation of this general property of learning.
    
    \begin{restatable}[Famine of Favorable Information Resources]{theorem}{fofir}
        Let $\mathcal{B}$ be a finite set of information resources and let $t \subseteq \Omega$ be an arbitrary fixed $k$-size target set with corresponding target function $\bm{t}$. Define 
        \begin{align*}
            %R &= \{f \mid f \in \mathcal{B} \}, \text{ and}
            %\\
            \mathcal{B}_{q_{\mathrm{min}}} &= \{f \mid f \in \mathcal{B}, q(t,f) \geq q_{\mathrm{min}} \},
        \end{align*}
        where $q(t,f)$ is the expected per-query probability of success for algorithm $\mathcal{A}$ on search problem $(\Omega, t,f)$ and $q_{\mathrm{min}} \in [0,1]$ represents the minimally acceptable per-query probability of success. Then,
        \begin{align*}
            \frac{|\mathcal{B}_{q_{\mathrm{min}}}|}{|\mathcal{B}|} &\leq \frac{p +  \bias(\mathcal{B}, \bm{t})}{q_{\mathrm{min}}}
        \end{align*}
        where $p = \frac{k}{|\Omega|}$.
        \label{thm:fofir}
    \end{restatable}
    \noindent
    This theorem shows us that unless our set of information resources is biased towards our target, only a small proportion of information resources will yield a high probability of search success. In most practical cases, $p$ is small enough that uniform random sampling is not considered a plausible strategy, since we typically have small targets embedded in large search spaces. Thus the bound is typically very constraining. The set of information resources will be overwhelmingly unhelpful unless we restrict the given information resources to be positively biased towards the specified target.
    
    \begin{restatable}[Proportion of Successful Problems Under Bias-Free Search]{corollary}{reducedproportion}
    When \(\bias(\mathcal{B}, \bm{t}) = 0\),
    \begin{align*}
        \frac{|\mathcal{B}_{q_{\mathrm{min}}}|}{|\mathcal{B}|} &\leq \frac{p}{q_{\mathrm{min}}}
    \end{align*}
    \label{cor:reducedproportion}
    \end{restatable}
    \noindent Directly following Theorem \ref{thm:fofir}, if the algorithm does not induce bias on $\bm{t}$ given a set of information resources, the proportion of successful search problems cannot be any higher than the single-query success probability of uniform random sampling divided by the minimum specified performance.
    
    \begin{restatable}[Futility of Bias-Free Search]{theorem}{futility}
    For any fixed algorithm $\mathcal{A}$, fixed target $t \subseteq \Omega$ with corresponding target function $\bm{t}$, and distribution over information resources $\mathcal{D}$, if $\bias(\mathcal{D}, \bm{t}) = 0$, then
    \begin{align*}
        \Pr(\omega \in t; \mathcal{A}) &= p
    \end{align*}
    where $\Pr(\omega \in t; \mathcal{A})$ represents the per-query probability of successfully sampling an element of $t$ using $\mathcal{A}$, marginalized over information resources $F \sim \mathcal{D}$, and $p$ is the single-query probability of success under uniform random sampling.
    \end{restatable}
    \noindent
    This result shows that without bias, an algorithm can perform no better than uniform random sampling. This is a generalization of Mitchell's idea of the futility of removing biases for binary classification \cite{needforbiases} and Monta\~nez's formal proof for the need for bias for multi-class classification \cite{montanez2017dissertation}. This result shows that bias is necessary for any machine learning or search problem to have better than random chance performance.
    
        \begin{restatable}[Famine of Applicable Targets]{theorem}{foat}
    Let $\mathcal{D}$ be a distribution over a finite set of information resources. Define
    \begin{align*}
        \tau_k &= \{t \mid t \subseteq \Omega, |t| = k\} \\
        \tau_{q_{\mathrm{min}}} &= \{t \mid t \in \tau_k, \bias(\mathcal{D}, \bm{t}) \geq q_{\mathrm{min}}\} 
    \end{align*}
    where $\bm{t}$ is the target function corresponding to the target set $t$. Then,
    \[
      \frac{|\tau_{q_\mathrm{min}}|}{|\tau_k|} \leq \frac{p}{p + q_\mathrm{min}} \leq \frac{p}{q_\mathrm{min}}
    \]
    where $p = \frac{k}{|\Omega|}$.
    \end{restatable}
    \noindent
    This theorem shows that the proportion of target sets for which our algorithm is highly biased is small, given that $p$ is small relative to $q_\mathrm{min}$. A high value of $\bias(\mathcal{D}, \bm{t})$ implies that the algorithm, given $\mathcal{D}$, places a large amount of mass on $\bm{t}$ and a small amount of mass on other target functions. Consequently, our algorithm is acceptably biased toward fewer target sets as we increase our minimum threshold of bias.
    
    \begin{restatable}[Famine of Favorable Biasing Distributions]{theorem}{fofbd}
      Given a fixed target function $\bm{t}$, a finite set of information resources $\mathcal{B}$, and a set $\mathcal{P} = \{\mathcal{D}\mid \mathcal{D} \in \mathbb{R}^{|\mathcal{B}|}, \sum_{f \in \mathcal{B}} \mathcal{D}(f) = 1 \}$ of all discrete $|\mathcal{B}|$-dimensional simplex vectors,
      \[
        \frac{\mu(\mathcal{G}_{\bm{t}, q_\mathrm{min}})}{\mu(\mathcal{P})} \leq \frac{p + \bias(\mathcal{B}, \bm{t})}{q_\mathrm{min}}
      \]
      where $\mathcal{G}_{\bm{t}, q_\mathrm{min}} = \{\mathcal{D} \mid \mathcal{D} \in \mathcal{P}, \bias(\mathcal{D}, \bm{t}) \geq q_\mathrm{min}\}$ and $\mu$ is Lebesgue measure.
    \end{restatable}
    \noindent
    We see that the proportion of distributions over $\mathcal{B}$ for which our algorithm is acceptably biased towards a fixed target function $\bm{t}$ decreases as we increase our minimum acceptable level of bias, $q_\mathrm{min}$. Additionally, the greater the amount of bias induced by our algorithm given a set of information resources on a fixed target, the higher the probability of identifying a suitable distribution that achieves successful search. However, unless the set is already filled with favorable elements, finding a minimally favorable distribution over that set is difficult.
    
    \begin{restatable}[Bias Over Distributions]{theorem}{density}
      Given a finite set of information resources $\mathcal{B}$, a fixed target function $\bm{t}$, and a set $\mathcal{P} = \{\mathcal{D}\mid \mathcal{D} \in \mathbb{R}^{|\mathcal{B}|}, \sum_{f \in \mathcal{B}} \mathcal{D}(f) = 1 \}$ of discrete $|\mathcal{B}|$-dimensional simplex vectors,
      \[
        \int_\mathcal{P} \bias(\mathcal {D}, \bm{t}) \dif\mathcal {D} = C \cdot \bias(\mathcal{B}, \bm{t})
      \]
      where $C = \int_\mathcal{P} \dif\mathcal {D}$ is the uniform measure of set $\mathcal{P}$. For an unbiased set $\mathcal{B}$,
      \[
        \int_\mathcal{P} \bias(\mathcal{D}, \bm{t}) \dif\mathcal {D} = 0
      \]
    \end{restatable}
    \noindent
    This theorem states that the total bias on a fixed target function over all possible distributions is proportional to the bias induced by the algorithm given $\mathcal{B}$. When there is no bias over a set of information resources, the total bias over all distributions sums to $0$. It follows that any distribution over $\mathcal{D}$ for which the algorithm places positive bias on $\bm{t}$ is offset by one or more for which the algorithm places negative bias on $\bm{t}$.
    
    \begin{restatable}[Conservation of Bias Over Distributions]{corollary}{conservationdistributions}
    Let $\tau_{k} = \{ \bm{t} | \bm{t} \in \{ 0, 1 \}^{ |\Omega| }, ||\bm{t}|| = \sqrt{k} \}$ be the set of all $|\Omega|$-length $k$-hot vectors. Then, \[\sum_{\bm{t} \in \tau_{k}} \int_{\mathcal{P}} \bias(\mathcal{D}, \bm{t}) \dif\mathcal{D} = 0\]
    \end{restatable}
    \noindent
    This result extends our conservation results, showing that the total bias over all distributions and all $k$-size target sets sums to zero, even when beginning with a set of information resources that is favorably biased towards a particular target.


==> old_proof.tex <==
Let 
    $f(x_1, \dots, x_n) = \frac{1}{n} \sum_{i = 1}^n \bm{t}^\top \overline{P}_{x_i}$.
    Swapping an element $x_i$ with an arbitrary element $x_{i'}$ can, in the most extreme case, transfer all of the probability mass to or from the target such that $|\bm{t}^\top \overline{P}_{x_i} -\bm{t}^\top \overline{P}_{x_{i'}}| = 1$. Then, 
    \begin{align*}
        \lub{x_1, \dots, x_n, x_{i'}} \hspace{-1em}|f(x_1, \dots, x_i,\dots,x_n) - f(x_1, \dots, x_{i'}, \dots,x_n)| &\leq \frac{1}{n}
    \end{align*}
    We seek to bound the probability of large differences between $\bias(X, t)$ and $\bias(\mathcal{D}, t)$, namely
    \begin{align*}
        & \mathbbm{P}(|\bias(X, \bm{t}) - \bias(\mathcal{D}, \bm{t})| \geq \epsilon)\\ 
            &= \mathbbm{P}(|\mathbbm{E}_{F \sim \mathcal{U}[X]}[\bm{t}^\top\overline{P}_F] - \mathbbm{E}_{F \sim \mathcal{D}}[\bm{t}^\top\overline{P}_F]| \geq \epsilon).
    \end{align*}
    By the law of iterated expectations, $$\mathbbm{E}_{F}[t^\top\overline{P}_F] = \mathbbm{E}_{X}[\mathbbm{E}_{F}[t^\top \overline{P}_F \mid  X]].$$ Continuing, 
    \begin{align*}
            & \mathbbm{P}(|\bias(X, \bm{t}) - \bias(\mathcal{D}, \bm{t})| \geq \epsilon) \\
            %&= \mathbbm{P}(\big|\mathbbm{E}_{F \sim \mathcal{U}[X]}[t^\top\overline{P}_F]
            %- \mathbbm{E}_{X \sim \mathcal{D}}[\mathbbm{E}_{F \sim \mathcal{U}[X]}[t^\top \overline{P}_F \mid X]]\big| \geq \epsilon) \\
            &= \mathbbm{P}(\big|\mathbbm{E}_{F}[\bm{t}^\top\overline{P}_F]
            - \mathbbm{E}_{X}[\mathbbm{E}_{F}[\bm{t}^\top\overline{P}_F \mid X]]\big| \geq \epsilon)\\
            &= \mathbbm{P}(\big|f(X) - \mathbbm{E}_{X}[f(X)]\big| \geq \epsilon)\\ 
            &\leq 2 e^{-2 n\epsilon^2},
    \end{align*}
    where the final inequality follows from McDiarmid's inequality.
